Perennial Semantic Data Terms of Use for Decentralized Web

In today's digital landscape, the Web has become increasingly centralized, raising concerns about user privacy violations. Decentralized Web architectures, such as Solid, offer a promising solution by empowering users with better control over their data in their personal `Pods'. However, a significant challenge remains: users must navigate numerous applications to decide which application can be trusted with access to their data Pods. This often involves reading lengthy and complex Terms of Use agreements, a process that users often find daunting or simply ignore. This compromises user autonomy and impedes detection of data misuse. We propose a novel formal description of Data Terms of Use (DToU), along with a DToU reasoner. Users and applications specify their own parts of the DToU policy with local knowledge, covering permissions, requirements, prohibitions and obligations. Automated reasoning verifies compliance, and also derives policies for output data. This constitutes a ``perennial'' DToU language, where the policy authoring only occurs once, and we can conduct ongoing automated checks across users, applications and activity cycles. Our solution is built on Turtle, Notation 3 and RDF Surfaces, for the language and the reasoning engine. It ensures seamless integration with other semantic tools for enhanced interoperability. We have successfully integrated this language into the Solid framework, and conducted performance benchmark. We believe this work demonstrates a practicality of a perennial DToU language and the potential of a paradigm shift to how users interact with data and applications in a decentralized Web, offering both improved privacy and usability.

==> 2-related-research-ver2.tex <==
% \subsection{Running case}

% To illustrate why existing languages are not appropriate to use in our targeted decentralized Web context, we present a realistic minimal example scenario here to illustrate the requirements for this context. Then, we will briefly discuss related existing languages.

% Alice is planning to use an online shopping app to buy shoes, and expects this app to read several types of data in her Pod: her foot size, delivery address, and billing information, each with different types of usage expectations.
% Her foot size can be read by any application for the purpose of shopping, product matching and doing recommendation; her delivery address is the full address, and can only be used for the purpose of sending parcels; her billing information is very sensitive, and can only be read for the purpose of making payments, and shared with banks also for the purpose of making payments only. 
% Now, Alice finds a shopping app, SmartShop, and wants to know whether she could use this app, e.g.~whether SmartShop complies with all the expected terms for her data.

% On the other hand, Bob, the developer of SmartShop is an ethical developer and wants to improve users' trust, so they will choose to use his app. Of course the users will not be able to examine the details of the app because it is proprietary, neither can the app be put into an isolated offline environment because it requires connection to external sources for lots of information. Bob can provide some descriptions on how the app processes different types of data, but he knows users normally will not read such descriptions because they are too long. Now Bob wants to know how to overcome this issue.


% Assume a user, Alice, is planning to use an online shopping app to buy shoes, and expects this app to read several types of data in her Pod: her foot size, delivery address, and billing information, each with different sensitivity levels and different types of usage expectations. Alice finds a shopping app, HappyShop, and wants to know whether she should use this app or not, particularly whether the app uses her data ethically.
% Apparently, it is infeasible or even impossible to require Alice to read the source code of HappyShop to make this decision.
% In the meantime, Bob, the developer of HappyShop, wants to improve users' trust so they will use his app, and is willing to present some high-level descriptions on how HappyShop treats data. Thus, Terms of Use emerges not only as a legal requirement, but also real-life necessities.
% However, it is also widely known that users do not read these terms (aka.~``the biggest lie on the Internet''), because of information overloading for the large number of such documents and the length and content of the documents []. With larger amount of applications in a decentralized Web, this issue can only become more prominent, and Alice will tend to forgo her right in the long run.
% It impairs the user autonomy promise of the decentralized Web if this remains the same, and will lead to many issues as already demonstrated in today's Web, from unable to proactively discover potential misuse of data [], to being over-cautious thus preventing rightful data usage [].

Several explorations have delved into the utilization of computer-interpretable formal encoding of policies to enable (semi-)automated decision-making of data usage authorization. These range from the classical access control to more advanced dynamic usage descriptions. In this section, we examine this body of research and discusses their relevance to a decentralized Web context%.
, in addition to Table \ref{tab:related_research_features} which summarizes their main features.

\begin{table*}[]
    \centering
    \caption{Summarization of features of related policy languages.}
    {\footnotesize  C1 - C5 refers to the Challenges 1 - 5 identified for perennial language. For column C1, A means authorization, O means obligation. For column C2, C means capacity, I means multi-input, M means use mode, P means purpose, T means data type/category. For column C3 \& C4, T means true, T(e) means true if using same environmental information schema. For column C5, O means multi-output, T means transformation. For column Condition, A means application, C means capacity, E means (common) environmental information, \textit{\textbf{E}} means Entire environmental information exposed in knowledge base, M means use mode, P means purpose, T means data type/category, U means user, X means external information.}
    \label{tab:related_research_features}
    
    \begin{tabular}{ccccccccc}
        \toprule
        Language & C1 & C2 & C3 & C4 & C5 & Condition & Policy Author & Format \\
        \midrule
        E-P3P\cite{karjoth_platform_2002} & AO &  & T & T(e) &  & UEP & Supervisor & Custom \\
        XACML\cite{noauthor_extensible_2013}/ODRL\cite{noauthor_odrl_2018} & AO+ &  & T & T(e) & & EPU & Owner & XMl/JSON-LD \\
        WAC\cite{noauthor_web_2022}/ACP\cite{noauthor_access_2022} & A & & T & & & AU/AUX & Owner & Turtle \\
        P2U\cite{iyilade_p2u_2014} & A & & T & & & AU & Owner & XML \\
        LaBAC\cite{biswas_label-based_2016} & A & & T & & & AU & Supervisor & Custom \\
        AIR\cite{kagal_using_2008} & A & & T & T(e) & & U\textit{\textbf{E}} & Owner & N3 \\
        Thoth\cite{elnikety_thoth_2016} & A & & T & & & EUX & Owner & Logic-like \\
        Eddy\cite{breaux_eddy_2014} & AO & MP &  & T(e) & T & MPU & Supervisor & OWL-DL  \\
        LoNet\cite{havard_d_johansen_enforcing_2015} & A & & T & T & T & EU & Supervisor & Custom \\
        CamFlow\cite{pasquier_camflow_2017} & A & C & T & T & T & C & Owner & Custom \\
        Smart object\cite{sagirlar_decentralizing_2018} & A & IPT & T & T & T & PT & Owner & Custom \\
        Dr.Aid\cite{rui_zhao_draid_2021} & AO & IP & T & T & OT & EPU & Owner & Custom 
        \vspace{0.3em} \\
        \textbf{Ours} & AO & ACIPT & T & T & OT & CEPU & Owner & Turtle \\
        \bottomrule
    \end{tabular}
\end{table*}

There are policy languages that utilize semantic technologies or are tailored for specific use cases within the decentralized Web. One notable example is the Open Digital Rights Language (ODRL)~\cite{noauthor_odrl_2018}, a well-known expressive policy language serializable to JSON-LD. It offers a comprehensive set of concepts, including permissions, prohibitions, obligations, remedies, conditions, purposes and agents. However, originated as a data right expression language, ODRL primarily focuses on expressing what is (not) permitted for the data, and lacks a corresponding mechanism for expressing application information. While efforts are being made to address this issue \cite{esteves_odrl_2021}, there is still uncertainty regarding the eventual resolution.
% the representation of much information is context-dependent, affecting the generality of the reasoner (validator).
The AIR \cite{kagal_using_2008} policy language, based on Notation 3 (N3) \cite{berners-lee_n3logic_2008}, specifies permitted and prohibited actions for data processing. It allows for the expression of custom rules directly on the contextual knowledge base of data processing. However, similar to ODRL, in the absence of general agreements across applications, this requires the policy author to have the knowledge of the information available in the knowledge base, resulting in a high level of coupling with the application.
Eddy \cite{breaux_eddy_2014} examined real-life terms of use from online services and proposed a policy language based on OWL-DL to express key data requirements, including permissions, obligations and prohibitions. The language distinguishes between different types of use modes (collect, use, retain and transfer) and demonstrated compliance checking between two policy sets of two services. However, there is no clear demonstration of how data providers can utilize this language, as it necessitates highly detailed descriptions.
Solid, a decentralized Web architecture based on Linked Data, has its own policy languages, mainly for access control purposes. This includes WAC \cite{noauthor_web_2022}, a policy language for expressing ACL, and ACP \cite{noauthor_access_2022}, an advanced policy language that supports a broad range of conditions, such as Verifiable Credentials. WAC and ACP leverage contextual information exposed by Solid but are less expressive compared to ODRL and AIR.
In general, these languages cannot be directly applied to support data usage expressions in the decentralized setting we target at due to their individual limitations. %In addition, there is no clear solution for associating policies with output data of the application, leading to an undesired impact for the interaction across applications if they share data.Reusing them would introduce heavy overload when designing a new language, though their expressiveness may be useful in the future when extending the language.

Apart from them, the most well-known line of research involves various access control models, each based on different principles. For example, models such as Mandatory Access Control (MAC) \cite{sandhu_access_1994}, Access Control List (ACL), Role-Based Access Control (RBAC) \cite{sandhu_role-based_1996} or Attribute-Based Access Control (ABAC), can be based on information ranging from narrower details like user identity to broader categories such as user groups, and contextual information. Several languages use or implement them, such as E-P3P \cite{karjoth_platform_2002}, WAC \cite{noauthor_web_2022}, P2U \cite{iyilade_p2u_2014}, XACML \cite{noauthor_extensible_2013} and ODRL \cite{noauthor_odrl_2018}. There is also research that falls in the middle ground, such as Label-Based Access Control (LaBAC) \cite{biswas_label-based_2016}, a simplified variant of ABAC while more expressive than MAC and RBAC, using simple tuples to express conditions on users, actions and data (objects).

% Other policy languages may also use the concepts from access models, with additional features, such as eXtensible Access Control Markup Language (XACML) \cite{noauthor_extensible_2013}, a widely-known XML-based standard for ABAC with additional constructs like obligations for cloud services, and ODRL \cite{noauthor_odrl_2018}, which will be discussed later.
Noticeably, eXtensible Access Control Markup Language (XACML) provides construct of 
In general, this type of research usually assumes a finite number of personnel (including applications) engaged in policy checking, and thus presupposes the presence of a `supervisor' with abundant knowledge to actively compile and maintain policies, particularly when there are personnel changes. While this assumption is reasonable for managing data usage at an institutional level, it presents challenges in contexts with multiple independent stakeholders that engage and disengage dynamically, as is the case in a decentralized Web.

Some other research also makes similar assumptions, but allows for customized mechanisms within their policies. For instance, P2U \cite{iyilade_p2u_2014}, a data-right language akin to a set  of contracts, defines permitted data usage activities for applications, data, users and meta-information (e.g.~``negotiable''). Thoth \cite{elnikety_thoth_2016}, on the other hand, uses its own logic-like policy language to express policies not only for read action, but also for write, update and declassification actions. It permits intricate evaluations of formulae that involve rich operators and the incorporation of external sources of information during policy evaluation. While these approaches vary in terms of expressiveness and usage contexts, they share a common limitation due to the assumption of a finite number of personnel. In our example, they can only define the policy \emph{after} a user like Alice has determined whether a shopping app like HappyShop should be granted permission or not, rather than proactively.

In contrast to the approaches mentioned above, some research recognizes the dynamic nature of data and applications, and offers different solutions. LoNet \cite{havard_d_johansen_enforcing_2015}, for example, employs Information Flow Control (IFC) for RBAC, along with special transformation rules for policy evolution. Additionally, it uses custom meta-code for checking additional policy information like time. However, the most expressive part, the meta-code, is arbitrary and difficult to statically verify.
CamFlow \cite{pasquier_camflow_2017}, on the other hand, borrows concepts from Decentralized IFC (DIFC) \cite{myers_decentralized_1997}, and employs homogeneous policy constructs (tags and labels) to encode the data policy and application capability, and checks their compatibility. It also allows the expression of policy evolution by adding or removing tags for output (policy) based on input (policy). 
Smart object \cite{sagirlar_decentralizing_2018} uses complex constructs to define permitted and prohibited use of data, and combines this with the application information (using relational calculus) to derive policies for output data, assuming and leveraging a tabular structure of data.
Dr.Aid \cite{rui_zhao_draid_2021} focuses on the context of data-intensive scientific workflows, employing different structures to express data rules and process rules. It supports policy reasoning and derivation for workflow graphs involving multiple processes.
A common feature among these approaches is the separation of data policy from application policy, using pre-defined reasoning mechanisms to facilitate compliance checking. They have demonstrated that this separation allows the reasoner to verify if an application complies with the data policy, aligning with our intended goal.



==> 2-related-research.tex <==


% \subsection{Running case}

% To illustrate why existing languages are not appropriate to use in our targeted decentralized Web context, we present a realistic minimal example scenario here to illustrate the requirements for this context. Then, we will briefly discuss related existing languages.

% Alice is planning to use an online shopping app to buy shoes, and expects this app to read several types of data in her Pod: her foot size, delivery address, and billing information, each with different types of usage expectations.
% Her foot size can be read by any application for the purpose of shopping, product matching and doing recommendation; her delivery address is the full address, and can only be used for the purpose of sending parcels; her billing information is very sensitive, and can only be read for the purpose of making payments, and shared with banks also for the purpose of making payments only. 
% Now, Alice finds a shopping app, SmartShop, and wants to know whether she could use this app, e.g.~whether SmartShop complies with all the expected terms for her data.

% On the other hand, Bob, the developer of SmartShop is an ethical developer and wants to improve users' trust, so they will choose to use his app. Of course the users will not be able to examine the details of the app because it is proprietary, neither can the app be put into an isolated offline environment because it requires connection to external sources for lots of information. Bob can provide some descriptions on how the app processes different types of data, but he knows users normally will not read such descriptions because they are too long. Now Bob wants to know how to overcome this issue.


% Assume a user, Alice, is planning to use an online shopping app to buy shoes, and expects this app to read several types of data in her Pod: her foot size, delivery address, and billing information, each with different sensitivity levels and different types of usage expectations. Alice finds a shopping app, HappyShop, and wants to know whether she should use this app or not, particularly whether the app uses her data ethically.
% Apparently, it is infeasible or even impossible to require Alice to read the source code of HappyShop to make this decision.
% In the meantime, Bob, the developer of HappyShop, wants to improve users' trust so they will use his app, and is willing to present some high-level descriptions on how HappyShop treats data. Thus, Terms of Use emerges not only as a legal requirement, but also real-life necessities.
% However, it is also widely known that users do not read these terms (aka.~``the biggest lie on the Internet''), because of information overloading for the large number of such documents and the length and content of the documents []. With larger amount of applications in a decentralized Web, this issue can only become more prominent, and Alice will tend to forgo her right in the long run.
% It impairs the user autonomy promise of the decentralized Web if this remains the same, and will lead to many issues as already demonstrated in today's Web, from unable to proactively discover potential misuse of data [], to being over-cautious thus preventing rightful data usage [].

Several explorations have delved into the utilization of computer-interpretable formal encoding of policies to enable (semi-)automated decision-making of data usage authorization. These range from the classical access control to more advanced dynamic usage descriptions. In this section, we examine this body of research and discusses their relevance to a decentralized Web context%.
, in addition to Table \ref{tab:related_research_features} which summarizes their main features (see Appendix \ref{sec:appendix:related-work-extension} for further details of term explanation).

\begin{table*}[ht]
    \centering
    \caption{Summarization of features under different categories of related policy languages.}
    {\footnotesize  C1 - C5 refers to the Challenges 1 - 5 identified for perennial language. For column C1, A means authorization, O means obligation, and + means additional features. For columns C3 \& C4, \checked~means true, \CheckedBox~means true if using same environmental information schema. For columns C2, C5 and Condition, A means application, C means capacity, D means data type / category, E means environmental information, \textit{\textbf{E}} means entire environmental information exposed in knowledge base, I means multi-input, M means use mode, O means multi-output, P means purpose, T means transformation, U means user, X means external information.}
    \label{tab:related_research_features}
    
    \begin{tabular}{ccccccccc}
        \toprule
        Language & C1 & C2 & C3 & C4 & C5 & Condition & Policy Author & Format \\
        \midrule
        E-P3P\cite{karjoth_platform_2002} & AO &  & \checked & \CheckedBox &  & EPU & Supervisor & Custom \\
        XACML\cite{noauthor_extensible_2013}/ODRL\cite{noauthor_odrl_2018} & AO+ &  & \checked & \CheckedBox & & EPU & Owner & XML/JSON-LD \\
        WAC\cite{noauthor_web_2022}/ACP\cite{noauthor_access_2022} & A & & \checked & & & AU/AUX & Owner & Turtle \\
        P2U\cite{iyilade_p2u_2014} & A & & \checked & & & AU & Owner & XML \\
        LaBAC\cite{biswas_label-based_2016} & A & & \checked & & & AU & Supervisor & Custom \\
        AIR\cite{kagal_using_2008} & A & & \checked & \CheckedBox & & \textit{\textbf{E}}U & Owner & N3 \\
        Thoth\cite{elnikety_thoth_2016} & A & & \checked & & & EUX & Owner & Logic-like \\
        Eddy\cite{breaux_eddy_2014} & AO & MP &  & \CheckedBox & T & MPU & Supervisor & OWL-DL  \\
        LoNet\cite{havard_d_johansen_enforcing_2015} & A & & \checked & \checked & T & EU & Supervisor & Custom \\
        CamFlow\cite{pasquier_camflow_2017} & A & C & \checked & \checked & T & C & Owner & Custom \\
        Smart object\cite{sagirlar_decentralizing_2018} & A & DIP & \checked & \checked & T & DP & Owner & Custom \\
        Dr.Aid\cite{rui_zhao_draid_2021} & AO & IP & \checked & \checked & OT & EPU & Owner & Custom 
        \vspace{0.3em} \\
        \textbf{This paper} & AO & CDIP & \checked & \checked & OT & CEPU & Owner & Turtle \\
        \bottomrule
    \end{tabular}
\end{table*}

The most well-known line of research involves various access control models, each based on different principles. For example, models such as Mandatory Access Control (MAC) \cite{sandhu_access_1994}, Access Control List (ACL), Role-Based Access Control (RBAC) \cite{sandhu_role-based_1996} or Attribute-Based Access Control (ABAC), can be based on information ranging from narrower details like user identity to broader categories such as user groups, and contextual information. Several languages uses or implements them, such as E-P3P \cite{karjoth_platform_2002}, WAC \cite{noauthor_web_2022} and P2U \cite{iyilade_p2u_2014}. There is also research that falls in the middle ground, such as Label-Based Access Control (LaBAC) \cite{biswas_label-based_2016}, a simplified variant of ABAC while more expressive than MAC and RBAC, using simple tuples to express conditions on users, actions and data (objects).

Other policy languages may also use the concepts from access models, with additional features, such as eXtensible Access Control Markup Language (XACML) \cite{noauthor_extensible_2013}, a widely-known XML-based standard for ABAC with additional constructs like obligations for cloud services, and ODRL \cite{noauthor_odrl_2018}, which will be discussed later.
In general, this type of research usually assumes a finite number of personnel (including applications) engaged in policy checking, and thus presupposes the presence of a `supervisor' with abundant knowledge to actively compile and maintain policies, particularly when there are personnel changes. While this assumption is reasonable for managing data usage at an institutional level, it presents challenges in contexts with multiple independent stakeholders that engage and disengage dynamically, as is the case in a decentralized Web.

Some other research also makes similar assumptions, but allows for customized mechanisms within their policies. For instance, P2U \cite{iyilade_p2u_2014}, a data-right language akin to a set  of contracts, defines permitted data usage activities for applications, data, users and meta-information (e.g.~``negotiable''). Thoth \cite{elnikety_thoth_2016}, on the other hand, uses its own logic-like policy language to express policies not only for read action, but also for write, update and declassification actions. It permits intricate evaluations of formulae that involve rich operators and the incorporation of external sources of information during policy evaluation. While these approaches vary in terms of expressiveness and usage contexts, they share a common limitation due to the assumption of a finite number of personnel. In our example, they can only define the policy \emph{after} a user like Alice has determined whether a shopping app like HappyShop should be granted permission or not, rather than proactively.

In contrast to the approaches mentioned above, some research recognizes the dynamic nature of data and applications, and offers different solutions. LoNet \cite{havard_d_johansen_enforcing_2015}, for example, employs Information Flow Control (IFC) for RBAC, along with special transformation rules for policy evolution. Additionally, it uses custom meta-code for checking additional policy information like time. However, the most expressive part, the meta-code, is arbitrary and difficult to statically verify.
CamFlow \cite{pasquier_camflow_2017}, on the other hand, borrows concepts from Decentralized IFC (DIFC) \cite{myers_decentralized_1997}, and employs homogeneous policy constructs (tags and labels) to encode the data policy and application capability, and checks their compatibility. It also allows the expression of policy evolution by adding or removing tags for output (policy) based on input (policy). 
Smart object \cite{sagirlar_decentralizing_2018} uses complex constructs to define permitted and prohibited use of data, and combines this with the application information (using relational calculus) to derive policies for output data, assuming and leveraging a tabular structure of data.
Dr.Aid \cite{rui_zhao_draid_2021} focuses on the context of data-intensive scientific workflows, employing different structures to express data rules and process rules. It supports policy reasoning and derivation for workflow graphs involving multiple processes.
A common feature among these approaches is the separation of data policy from application policy, using pre-defined reasoning mechanisms to facilitate compliance checking. They have demonstrated that this separation allows the reasoner to verify if an application complies with the data policy, aligning with our intended goal.

There are also policy languages that utilize semantic technologies or are tailored for specific use cases within the decentralized Web. One notable example is the Open Digital Rights Language (ODRL)~\cite{noauthor_odrl_2018}, a well-known expressive policy language serializable to JSON-LD. It offers a comprehensive set of concepts, including permissions, prohibitions, obligations, remedies, conditions, purposes and agents. However, originated as a data right expression language, ODRL primarily focuses on expressing what is (not) permitted for the data, and lacks a corresponding mechanism for expressing application information. While efforts are being made to address this issue \cite{esteves_odrl_2021}, there is still uncertainty regarding the eventual resolution.
% the representation of much information is context-dependent, affecting the generality of the reasoner (validator).
The AIR \cite{kagal_using_2008} policy language, based on Notation 3 (N3) \cite{berners-lee_n3logic_2008}, specifies permitted and prohibited actions for data processing. It allows for the expression of custom rules directly on the contextual knowledge base of data processing. However, in the absence of general agreements across applications, this requires the policy author to have the knowledge of the information available in the knowledge base, resulting in a high level of coupling with the application.
Eddy \cite{breaux_eddy_2014} examined real-life terms of use from online services and proposed a policy language based on OWL-DL to express key data requirements, including permissions, obligations and prohibitions. The language distinguishes between different types of data actions (collect, use, retain and transfer) and demonstrated compliance checking between two policy sets of two services. However, there is no clear demonstration of how data providers can utilize this language, as it necessitates highly detailed descriptions.
Solid, a decentralized Web architecture based on Linked Data, has its own policy languages, mainly for access control purposes. This includes WAC \cite{noauthor_web_2022}, a policy language for expressing ACL, and ACP \cite{noauthor_access_2022}, an advanced policy language that supports a broad range of conditions, such as Verifiable Credentials. WAC and ACP leverage contextual information exposed by Solid but are less expressive compared to ODRL and AIR.
In general, these languages cannot be directly applied to support data usage expressions in the decentralized setting we target at due to their individual limitations. %In addition, there is no clear solution for associating policies with output data of the application, leading to an undesired impact for the interaction across applications if they share data.Reusing them would introduce heavy overload when designing a new language, though their expressiveness may be useful in the future when extending the language.

% , but they do not fit with our target context in two reasons. First, Alice cannot know if she should use HappyShop, but can only know if using HappyShop complies with her policies. The subtle difference is that if noncompliance is found, Alice 

% There are also languages not belonging to the previous categories.
% For example, LoNet \cite{havard_d_johansen_enforcing_2015} is a hybrid between the first two types of research above, which uses IFC for RBAC, special transformation rules for policy evolution, and custom meta-code for checking additional types of information (e.g.~time). However, the most expressive part, meta-code, is arbitrary code and is hard to be statically checked.

% In summary, the various policy languages exhibit different features tailored for their specific use cases. Among them, we find the second category of research, which separates data policy from application policy, to be the most suitable for our intended design context.
% However, the existing languages in this category are not directly applicable to our context, primarily due to limitations in their exzpressiveness. For example, the tags of CamFlow are rudimentary and struggle to convey contextual information effectively. Smart Object enforces a rigid tabular structure of data, and offers limited support for conditions based on data category and usage purposes. Dr.Aid,  on the other hand,  primarily supports obligations and simulated prohibitions, with only limited expressions related to applications.
% Our research aims to address these limitations, and provide more constructs than both CamFlow and Dr.Aid in an expressive and extensible way.
